Generative Anomaly Detection for Time Series Datasets

Traffic congestion anomaly detection is of paramount importance in intelligent traffic systems. The goals of transportation agencies are two-fold: to monitor the general traffic conditions in the area of interest and to locate road segments under abnormal congestion states. Modeling congestion patterns can achieve these goals for citywide roadways, which amounts to learning the distribution of multivariate time series (MTS). However, existing works are either not scalable or unable to capture the spatial-temporal information in MTS simultaneously. To this end, we propose a principled and comprehensive framework consisting of a data-driven generative approach that can perform tractable density estimation for detecting traffic anomalies. Our approach first clusters segments in the feature space and then uses conditional normalizing flow to identify anomalous temporal snapshots at the cluster level in an unsupervised setting. Then, we identify anomalies at the segment level by using a kernel density estimator on the anomalous cluster. Extensive experiments on synthetic datasets show that our approach significantly outperforms several state-of-the-art congestion anomaly detection and diagnosis methods in terms of Recall and F1-Score. We also use the generative model to sample labeled data, which can train classifiers in a supervised setting, alleviating the lack of labeled data for anomaly detection in sparse settings.

==> experiments/classification.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[htb]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\hline
cluster                                                        & A & B & C & D & E & F & G & H \\ \hline
\begin{tabular}[c]{@{}l@{}}AUC\end{tabular} & 0.58 & 0.78 & 0.63 & 0.77 & 0.85 & 0.77 & 0.81 & 0.70 \\ \hline
\end{tabular}%
}
\caption{Avg AUC score for the MLPClassifier on 5 repeatedly generated synthetic test datasets.}
\label{tab:classification}
\end{table}

==> experiments/diagnosis_time.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[htb]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\hline
cluster                                                        & A & B & C & D & E & F & G & H \\ \hline
\begin{tabular}[c]{@{}l@{}}diagnosis \\ time (ms)\end{tabular} & 44.74 & 61.61 & 43.95 & 46.60 & 10.22 & 11.83 & 52.39 & 7.44 \\ \hline
\end{tabular}%
}
\caption{The average road segment-level anomaly diagnosis time for a particular anomalous timestamp over 5 runs with $\alpha=5\%$ and $\beta=50\%$.}
\label{tab:diagnosis_time}
\end{table}
